Achieving Spectrum Efficient Communication Under Cross-Technology Interference

In wireless communication, heterogeneous technologies such as WiFi, ZigBee and BlueTooth operate in the same ISM band.With the exponential growth in the number of wireless devices, the ISM band becomes more and more crowded. These heterogeneous devices have to compete with each other to access spectrum resources, generating cross-technology interference (CTI). Since CTI may destroy wireless communication, this field is facing an urgent and challenging need to investigate spectrum efficiency under CTI. In this paper, we introduce a novel framework to address this problem from two aspects. On the one hand, from the perspective of each communication technology itself, we propose novel channel/link models to capture the channel/link status under CTI. On the other hand, we investigate spectrum efficiency from the perspective by taking all heterogeneous technologies as a whole and building crosstechnology communication among them. The capability of direct communication among heterogeneous devices brings great opportunities to harmoniously sharing the spectrum with collaboration rather than competition.

==> Sec5_InterferenceM.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.45\textwidth]{cti.eps}
\caption{The Overview of CTI Modeling and Applications}
\label{ctioverview}
\end{figure}

\section{CTI Modeling and Applications}\label{sec:Main}
This section provides the overview of CTI modeling and its applications. 
As shown in Figure~\ref{ctioverview}, our designs sense the interference from heterogeneous devices 
such as WiFi, BlueTooth, and ZigBee. We then build CTI models, i.e., CTI 
detection, differentiation, and filtration models.
These CTI models have broad applications. For example, the accurate 
detection of CTI can help us design reliable spectrum access control mechanism. 
The interference detection, differentiation, and filtration information can also 
help us detect and recover corrupted symbols.

In the following of this section, we first introduces some preliminary about CTI modeling. 
Then we provides an overview of CTI models, followed by their applications.

\subsection{Preliminary}
When two wireless signals $X[n]$ and $Z[n]$ collide in the air, the receiver will receive the corrupted signals $Y[n]$ which is given by
\begin{equation}\label{equ:zigbeeinterfer}
\begin{array}{rcl}
Y[n] & = & H_{X}X[n] + H_ZZ[n] + W\vspace{0.15cm} \\
    & = & Y_X[n] + Y_Z[n] + W.
\end{array}
\end{equation}


After quadrature demodulation, the I(Q) samples of the $Y[n]$ are the results of low-pass filter when
multiplying $Y[n]$ by $cos(2\pi fn)$($-sin(2\pi fn)$) where $f$ is the center frequency of the carrier.
Therefore, we can get the following relation among the collided signals $Y_{I/Q}[n]$, the interference signals
$X_{I/Q}[n]$ and the original Zigbee signals $Z_{I/Q}[n]$.
\begin{equation}\label{equ:interfer}
\begin{array}{rcl}
Y_{I/Q}[n] = & LPF(Y_X[n]e^{-j2\pi fn}) \\
&+ LPF(Y_Z[n]e^{-j2\pi f n}) + W^\prime\\
          = & X_{I/Q}[n] + Z_{I/Q}[n] +  W^\prime.
\end{array}
\end{equation}

Actually, it is such addition relation on the I/Q samples to cause the differences among different interferences.
For example, if two ZigBee communications collide, the I/Q samples of corrupted symbols are the
addition of original correct signals, so the ZigBee interfered signals will show something
which only belonging to the correct ZigBee signals. While the interfered ZigBee signals corrupted by WiFi OFDM interference
may show some randomness in the RSSI of I/Q samples because of the accumulation of multiple sub-carriers. This is exactly the reason
why BeeShark can differentiate the wireless interference by mining the features of the signals of the corrupted ZigBee symbols.

\subsection{CTI Modeling}
This subsection introduces how to (i) detect, (ii) differentiate and (iii) filtrate
cross-technology interference.

\subsubsection{CTI Detection}
When a ZigBee receiver decodes out a packet shown in Figure \ref{fig:corruptpacket}, it
knew that the packet is corrupted after cyclic redundancy checking, but what
happened in detail? Using the hints provided by the physical layer interface, two parts of the packet
can be identified by the PPR\cite{PPR}, a classic work in this field,
the correct section including a correct packet header and
some packet content, i.e., the `11's in Figure \ref{fig:corruptpacket} and a
corrupted section from `E1' to the end can be identified successfully.
But for the question that the corruption from `E1' to the end are all come from the wireless
interference? PPR\cite{PPR} can't work anymore.

The hamming distances between the received chip sequence and the benchmark sequences
of the symbols are used to decode the packet at receivers, and the symbol with the minimum
hamming distance is the result of the decoder. If the the symbol is corrupted,
the received chip sequence will be hugely different from all the benchmark sequences.
So if the minimum hamming distance is above some threshold, we can determine that the received symbol is corrupted,
which is a normal way used to detect the corrupted symbols in many literatures such as PPR\cite{PPR}.

However, the detection of corrupted symbols is not the same thing as
the detection of interference. For example, there is a dramatic difference in the
signals for the different sections of corrupted symbols in the real packet
shown in Figure \ref{fig:corruptpacket}.

\begin{figure}[!htb]
\centering
\subfigure[After investigation by PPR]{
\label{fig:corruptpacket}
\includegraphics[width=0.23\textwidth]{Figures/corruptpacket.eps}}
\subfigure[After interference detection]{
\label{fig:detectpacket}
\includegraphics[width=0.23\textwidth]{Figures/detectpacket.eps}}
%\vspace{-4mm}
\caption{An instance of ZigBee packet with interference detection}
\label{fig:packets}
%\vspace{-4mm}
\end{figure}

%\begin{figure}[htbp]
%\centering
%\subfloat[After investigation by PPR\cite{PPR}]{\includegraphics[width=1.2in]{Figures/corruptpacket.eps}
%\label{fig:corruptpacket}}
%~~~~
%\subfloat[After interference detection]{\includegraphics[width=1.2in]{Figures/detectpacket.eps}
%\label{fig:detectpacket}}
%\caption{An instance of ZigBee packet with interference detection}
%\label{fig:packets}
%\end{figure}

Comparing the corrupted signals with the correct signal, the corrupted signals caused by wireless
interference will show much more randomness,
while there is an obvious shift for the corrupted signals for some internal corruption.
Such shift is caused by lack of time synchronization actually.
In fact, the packet will become a sequence of complex samples separated by some period after modulation and these
discrete values will be interpolated into a continuous signal for RF transmission.
At the receiver, this continuous signal should be sampled at the exact same positions
at the sender were. Due to lack of synchronization, a receiver cannot sample the received signal
exactly at the right positions, so some synchronization errors appear\cite{ZigZag}.

The difference between synchronization errors and wireless interferences can be identified
via more concrete physical soft hints. For example, the demodulation of ZigBee is based on
the phase shifts between consecutive samples, so the phase shifts are such soft hints.
Without wireless interference, some synchronization errors, such as sampling offset causes
little vibration or some fixed movements on such phase shifts, instead,
the phase shifts of the signals corrupted by CTIs show much more randomness. Therefore,
these features of phase shifts can be utilized to implement CTI detection.

\subsubsection{CTI Differentiation}
When two specific signals interfere, the interfered segments of the received signal
will show some unique features comparing with another two collided signals.
Specifically, when the I, Q values of the ZigBee signals, i.e., $I_Z$ and $Q_Z$ are collided with the
I, Q values of the interference signals, $I_X$ and $Q_X$, the RSSI of the corrupted signals will be:
\begin{equation}\label{equ:rssi}
\begin{array}{rcl}
RSSI & = & (I_Z+I_X)^2 + (Q_Z+Q_X)^2\vspace{0.15cm}\\

         & = & C + I_X^2 + Q_X^2 + \epsilon.
\end{array}
\end{equation}
The $I_Z^2 + Q_Z^2$ will be turned into a constant $C$ because of the half-sine pulses and $\pi/2$ offset between I and Q in the OQPSK modulation of ZigBees.

On the other hand, the cross terms in RSSI, i.e., $2I_ZI_X + 2Q_ZQ_X$ will
be approaching to the 0, as a result of the fact that the chips of ZigBee modulation come from some
pseudo-random sequences. Therefore, from the features of the interfered signals' RSSI, we can mining some
information about source of the wireless interferences.

For each symbol of WiFi 802.11b signals, the differential binary phase-shift keying (DBPSK) or differential
quadrature phase-shift keying (DQPSK) will produce the same RSSIs.
So the RSSI of interfered signals caused by 802.11b will show some periodicity after sampling.
While for WiFi 802.11g, the Orthogonal Frequency Division Multiplexing (OFDM) modulation
will make the corrupted signals are a sum of the signals on some orthogonal sub-carriers.
The unpredictable construction and destruction from different sub-carriers unlikely produce
a periodic RSSIs. So this feature of RSSIs in the interfered signals can be used to differentiate
the 802.11b or 802.11g CTIs. An example of such differentiation is shown in Figure \ref{fig:diffpacket}.

Moreover, the addition relation represented as formula (\ref{equ:interfer}) can also
result into some feature on the distribution of the phase shifts which are calculated as the
included angles formed by consecutive (I, Q) samples. Such difference in distribution
of phase shifts can differentiate the BlueTooth CTI.

\subsubsection{CTI Filtration}
Because most wireless communications use the quadrature modulation/demodulation to implement
the convert between the baseband signals and passband waveforms.
The samples of CTI signals are the addition of two type of wireless signals, or mathematically
\begin{equation}\label{equ:wirelessinfer}
I^{(F)}_i = I^{(T)}_i + \mathcal{W}_i, 1\leq i \leq 64,
\end{equation}
where $I^{(F)}_i$ means the $i^{th}$ corrupted (False) sample, $I^{(T)}_i$ is the
correct (True) sample and $\mathcal{W}_i$ denotes the signals introduced by wireless interference
at the $i^{th}$ sampling position.

Compared with original ZigBee signals, the signals come from
the wireless interference show out the obvious randomness, so the $\mathcal{W}_i$ in
formula (\ref{equ:wirelessinfer}) can be treated as a random noise.
Just based on the similar facts, the CrossZig combats the WiFi interference
by adding the multiple retransmission ZigBee signals\cite{CrossZig}.

Retransmission means same $I^{(T)}_i$s and different $\mathcal{W}_i$s, so the addition
can strengthen the inherent ZigBee signals and weaken the WiFi interference as well.
Enlightened by CrossZig, some partial interferences caused by CTIs can be filtered out by using the
information of the source of CTIs. More specifically, after some statistical filtration,
partial ZigBee symbols interfered by WiFi 802.11g signals can be recovered
illustrated in Figure \ref{fig:filterpacket}.

\begin{figure}[!htb]
\centering
\subfigure[After interference differentiation]{
\label{fig:diffpacket}
\includegraphics[width=0.23\textwidth]{Figures/diffpacket.eps}}
\subfigure[After interference detection]{
\label{fig:dectpacket}
\includegraphics[width=0.23\textwidth]{Figures/filterpacket.eps}}
%\vspace{-4mm}
\caption{An instance of ZigBee packet with interference differentiation and filtration}
\label{fig:filterpacket}
%\vspace{-4mm}
\end{figure}

%\begin{figure}[htbp]
%\centering
%\subfloat[After interference differentiation]{\includegraphics[width=1.2in]{Figures/diffpacket.eps}
%\label{fig:diffpacket}}
%~~~~
%\subfloat[After interference filtration]{\includegraphics[width=1.2in]{Figures/filterpacket.eps}
%\label{fig:dectpacket}}
%\caption{An instance of ZigBee packet with interference differentiation and filtration}
%\label{fig:filterpacket}
%\end{figure}

\subsection{Potential Applications}

Detecting the interference from heterogeneous devices can help us identify and recover
corrupted symbols (i.e., a basic unit of wireless transmission) caused by different sources
of interference. In detail, through CIT modeling, we can differentiate that a segment of
corrupted symbols is interfered by WiFi 802.11b transmissions while another segment is caused
by other hidden ZigBee terminals. Once interference is detected and differentiated, some
appropriate actions can be taken. For example, adaptive media access control protocols can
be called to respond the current wireless environment immediately and accurately.

On the other hand, once the source of interference is detected and identified successfully, this
knowledge can be used to recover the corrupted symbols and improve the wireless performance.
For example, partial retransmission or selective retransmission can be implemented to recover
the corrupted symbols and thus reducing the communication load. 

==> sec6_CTC_zm.tex <==
\section{Collaborative Cross-Technology Communication}\label{sec:Test}


In this section, we will discuss the concept, benefits and the establishment of the
cross-technology communication (CTC), i.e. the possible collaboration between heterogeneous devices, which is different from previous discussed cross-technology interference.


\subsection{Introduction to Cross-technology Communication (CTC)}

Previous link model and the interference detection methods aim at providing a co-existence scheme between multiple heterogeneous devices while requiring no or little modification to the existing standard hardware. However, these approaches inevitably suffer the fairness issue, since the sensing algorithm is usually implemented on the low-power devices. Different from the previous interference model, it is also possible to build direct communication between heterogeneous devices, while avoiding the modification of existing hardware.

Cross-technology communication (CTC) is one approach to provide direct communication between heterogeneous devices. CTC relies on the channel sensing mechanism, which is a must for many MAC protocols, such as CSMA. By sensing the channel energy (RSSI), receivers can sense the energy pattern generated by the sender, although it cannot demodulate the signal directly. In this way, CTC provide a way of direct communication for supporting advanced collaborative applications in IoT. The detailed benefits and the possible methods will be discussed in the later part of this section.


\subsection{Benefits}
To begin with, we introduce the examples of gains by enabling CTC, such as the cost, the channel efficiency and the applications.



\noindent \textbf{IoT Applications}
In the current deployed IoT systems, they require the deployment of multi-radio gateways as a bridge between heterogenous devices, which will take the message from one wireless protocol as the input, interpret the message into another wireless protocl, and then transmit the data int the air. The multi-radio gateway costs additional money, such as \$100.


In contrast, CTC builds directy Device-to-Devive (D2D) links between heterogeneous devices, without the requirement of the multiple-radio gateways. In this way, CTC reduces the cost of many IoT applications, such as the managemetn system in the warehouse and the home maintenance. For example, in the automatic home application, the WiFi AP collects the rain forecast in the next few hours
from the Internet, and sends this information to sprinklers equipped with the ZigBee sensros. The CTC enables the sprinklers to adjust the water consumption based on the raining condition in the future to save the water supply while providing the same maintaince.






\noindent \textbf{Energy savings}
As the low power devies, ZigBee sensors cost little energy compared with the energy consuming devices, such as WiFi. To save the energy, the WiFi radios can embed a seconday ZigBee radio to detec the messages from the nearby WiFi APs. In this way, the WiFi radios can be closed, and opened once the secondardy ZigBee radio detects an availble WiFi SSID.





\noindent \textbf{channel coordination}
To accomodate the wireless transmission between different senders, WiFi utilizes a RTS/CTS approach, which broadcasts the future channel status so that other senders remain silent during this duration. Similar to this iedea, it is possible to build a global RTS/CTS approach between heterogeneous devices. For example, a WiFi device which has a lot of traffic can broadcast the future channel status to the air, so taht the low-power ZigBee devices are able to delay their transmission. This global RTS/CTS approach can efficiently allocate the channel, and avoid the interference from the high power protocols on the low power protocols.






\subsection{Methods}
As CTC avoids the change of the hardware, it is currently built upon the channel sensing capability.


Different kinds of CTC:
[1] CTC via generated traffic
esense
howies
gsense (preamble require hardware modification)

[2] CTC via existing opportunity
freebee
Cmorse
N2W2, multiple communication directions



